Error Analysis of Sampling Algorithms for Approximating Stochastic Optimal Control

This paper is concerned with the error analysis of two types of sampling algorithms, namely model predictive path integral (MPPI) and an interacting particle system (\IPS) algorithm, that have been proposed in the literature for numerical approximation of the stochastic optimal control. The analysis is presented through the lens of Gibbs variational principle. For an illustrative example of a single-stage stochastic optimal control problem, analytical expressions for approximation error and scaling laws, with respect to the state dimension and sample size, are derived. The analytical results are illustrated with numerical simulations.

==> _definitions.tex <==
%%%spm macros %%%
\newcommand{\lr}[2]{\langle #1, #2 \rangle}
%\newcommand{\TepsN}{{{T}^{(N)}_\epsilon}}

\renewcommand{\em}{\it}
\def\fee{\upphi}
\newcommand{\RU}{R}
\newcommand{\RUinv}{\RU^{-1}}
\newcommand{\Ybar}{\bar{X}}
\renewcommand{\k}{{\sf K}}
\newcommand{\K}{{\sf K}}
\newcommand{\etabar}{{\eta}}
\newcommand{\newP}[1]{\noindent{\bf #1:}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\ud}{\mathrm{d}}
\def\Re{\mathbb{R}}
\def\R{\mathbb{R}}
\def\argmin{\mathop{\text{\rm arg\,min}}}
\def\argmax{\mathop{\text{\rm arg\,max}}}
\def\ind{\text{\rm\large 1}}
\def\varble{\,\cdot\,}
%This is p_n: \def\pxzn{p_{\text{\tiny$ X| Z^n$}}}
\newcommand{\Real}{\mathbb R}
\def\pop{\hbox{\tiny (POP)}}
\def\Lemma#1{Lemma~\ref{#1}}
\def\Proposition#1{Prop.~\ref{#1}}
\def\Theorem#1{Thm.~\ref{#1}}
\def\Corollary#1{Cor.~\ref{#1}}
\def\Sec#1{Sec.~\ref{#1}}
\def\Fig#1{Fig.~\ref{#1}}
\def\Appendix#1{Appendix.~\ref{#1}}
\newcommand{\tr}{\mathrm{tr}}
\def\eqdef{\mathrel{:=}}
\def\defeq{\mathrel{=:}}
\def\transpose{{\hbox{\rm\tiny T}}}
\def\clB{{\cal B}}
\def\clE{{\cal E}}
\def\clL{{\cal L}}
\def\clP{{\cal P}}
\def\clZ{{\cal Z}}
\def\clZd{{\cal Z}^{{}\, \hbox{\tiny $\blacksquare$}}}
\def\clW{{\cal W}}
\def\bfmX{\bfmath{X}}
\def\bfmZ{\bfmath{Z}}
\def\bfmU{\bfmath{U}}
\def\bfxi{\bfmath{xi}}
\newcommand{\E}[1]{\mathbb{E}[#1]}
\def\expect{{\sf E}}
\def\Expect{{\sf E}}
\def\clC{{\cal C}}
\def\clX{{\cal X}}
\def\Prob{{\sf P}}
\def\Probsub{{\sf P\! }}
\def\pgm#1{\notes{\textcolor{blue}{PGM: #1}}}
\def\P{{\sf P}}
\newcommand{\indicator}[1]{\mathbf{1}_{\left[ {#1} \right] }}
\newcommand{\cov}{\text{Cov}}
\newcommand{\backward}[1]{\overset{\shortleftarrow}{#1}}
\newcommand{\Ybarbar}{{Y}}
\newcommand{\SN}{S^{(N)}}
\def\Sec#1{Sec.~\ref{#1}}
\def\Thm#1{Thm.~\ref{#1}}
\def\Prop#1{Prop.~\ref{#1}}
%\newtheorem{theorem}{Theorem}
%\newtheorem{example}{Example}
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{remark}{Remark}
%\newtheorem{proposition}{Proposition}
%\newtheorem{corollary}{Corollary}
%\numberwithin{theorem}{chapter}
%\numberwithin{proposition}{chapter}
%\numberwithin{corollary}{chapter}
%\numberwithin{remark}{chapter}
%\numberwithin{lemma}{chapter}
%\numberwithin{example}{chapter}
%\numberwithin{definition}{chapter}
\newcommand{\pibar}{{\bar \pi}}
\newcommand{\trace}{\text{Tr}}
\newcommand{\val}{\tilde{\phi}}
\newcommand{\phiN}{\phi^{(N)}}
\newcommand{\kepsnorm}{{k}^{(\epsilon)}}
\newcommand{\kepsnormN}{{k}^{(\epsilon,N)}}
\newcommand{\kepsnormNN}{\bar{k}^{(\epsilon,N_2)}}
\newcommand{\keps}{{k}_{\epsilon}}
\newcommand{\kepsN}{{k}_{\epsilon}^{(N)}}
\newcommand{\Keps}{{K}_\epsilon}
\newcommand{\KepsN}{{K}_\epsilon^{(N)}}
\newcommand{\Kepsnorm}{\bar{K}_\epsilon}
\newcommand{\KepsnormN}{\bar{K}_\epsilon^{(N)}}
\newcommand{\phiepsN}{{\phi}^{(N)}_\epsilon}
\newcommand{\phieps}{{\phi}_{\epsilon}}
\newcommand{\LepsN}{{L}_\epsilon^{(N)}}
\newcommand{\HH}{H^1_0}
\newcommand{\sumiN}{\sum_{i=1}^N}
\newcommand{\phiM}{\phi^{(M)}}
\newcommand{\phiMN}{\phi^{(M,N)}}
\newcommand{\Deltaeps}{{\Delta_\rho}^{(\epsilon)}}
\newcommand{\DeltaepsN}{{\Delta_\rho}^{(\epsilon,N)}}
\newcommand{\rhoepsN}{\rho_\epsilon^{(N)}}
\newcommand{\rhoeps}{\rho^{(\epsilon)}}
\newcommand{\Teps}{{T}_{\epsilon}}
\newcommand{\Aeps}{{A}^{(\epsilon)}}
\newcommand{\TepsN}{{{T}^{(N)}_\epsilon}}
\newcommand{\mueps}{{\mu}^{(\epsilon)}}
\newcommand{\geps}{{g}_{\epsilon}}
\newcommand{\pr}{\rho}
\newcommand{\neps}{{n}_{\epsilon}}
\newcommand{\Ltwoeps}{{L^2_0(\mueps)}}
\newcommand{\FF}{C_0(\Omega)}
\newcommand{\infnorm}[1]{\|#1\|_\infty}
\newcommand{\PhiepsN}{{\Phi}^{(\epsilon,N)}}
\newcommand{\vepsN}{{{\sf K}}_\epsilon^{(N)}}
%\floatname{algorithm}{Procedure}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\Geps}{{G}_\epsilon}
\newcommand{\GepsN}{{G}_\epsilon^{(N)}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\Km}{{\bf K}}
\newcommand{\epsbar}{\bar{\epsilon}}
\newcommand{\meas}{\mu}
\newcommand{\aht}[1]{{\color{red} \text{#1}}}
\newcommand{\mN}{m^{(N)}}
\newcommand{\SigN}{\Sigma^{(N)}}
\newcommand{\GammaN}{\Gamma^{(N)}}
\newcommand{\OmegaN}{\Omega^{(N)}}
\newcommand{\snorm}[1]{\|#1\|_s}
\newcommand{\Fnorm}[1]{\|#1\|_F}
\newcommand{\Xs}{\bar{X}}
\newcounter{rmnum}




\newenvironment{romannum}{\begin{list}{{\upshape (\roman{rmnum})}}{\usecounter{rmnum}
\setlength{\leftmargin}{36pt}
\setlength{\rightmargin}{8pt}
\setlength{\itemsep}{2pt}
\setlength{\itemindent}{-1pt}
}}{\end{list}}

\newcounter{anum}
\newenvironment{alphanum}{\begin{list}{{\upshape (\alph{anum})}}{\usecounter{anum}
\setlength{\leftmargin}{14pt}
\setlength{\rightmargin}{8pt}
\setlength{\itemsep}{2pt}
\setlength{\itemindent}{-1pt}
}}{\end{list}}

\newcommand{\Ten}{{\sf T}}
\newcommand{\preps}{\pr_\epsilon}
\newcommand{\barphieps}{\bar{\phi}_\epsilon}
\newcommand{\barphiepsN}{\bar{\phi}_\epsilon^{(N)}}
\newcommand{\barnepsN}{\bar{n}_\epsilon^{(N)}}
\newcommand{\nepsN}{{n}_\epsilon^{(N)}}
\newcommand{\barkeps}{\bar{k}_\epsilon}
\newcommand{\barphivec}{\bar{{\sf  \Phi }}}
\newcommand{\barTen}{\bar{\sf T}}
\newcommand{\hvec}{{\sf h}}
\newcommand{\phivec}{{\sf \Phi}}

% Optimal transport FPF
\newcommand{\Xbar}{\bar{X}}
\newcommand{\PP}{{\sf P}}
\newcommand{\NN}{\mathcal{N}}
\def\Kbar{\bar{\sf K}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\tn}{_{t_{n}}}
\newcommand{\tnn}{_{t_{n-1}}}
\newcommand{\Sigmabar}{\bar{\Sigma}}
\newcommand{\var}{\text{Var}}
\newcommand{\X}{X}
\newcommand{\sRicc}{\sqrt{\text{Ricc}}}
\newcommand{\Ricc}{\text{Ricc}}
\newcommand{\ii}{k}
\def\FRAC#1#2#3{\genfrac{}{}{}{#1}{#2}{#3}}
\def\half{{\mathchoice{\FRAC{1}{1}{2}}%
		{\FRAC{2}{1}{2}}%
		{\FRAC{3}{1}{2}}%
		{\FRAC{4}{1}{2}}}}
	
\newcommand{\calN}{\mathcal{N}}
\newcommand{\hhat}{\hat{h}}

\newcommand{\Gdelta}{G^{(\delta)}}
\newcommand{\CA}{C_1}
\newcommand{\CB}{C_2}
\newcommand{\Ueps}{U_\epsilon}

\newcommand{\qeps}{q_\epsilon}
\newcommand{\qepsN}{q_\epsilon^{(N)}}


\newcommand{\Tan}{\text{Tan}}
\newcommand{\Id}{\text{Id}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calP}{\mathcal{P}}

\newcommand{\Pspace}{{\cal P}_{\text{ac},2}}
\newcommand{\LX}{{\sf L}}
\newcommand{\LP}{{\cal L}}
\newcommand{\HP}{{\cal H}}
\newcommand{\HX}{{\sf H}}
\newcommand{\JX}{{\sf J}}
\newcommand{\JP}{{\cal J}}
\newcommand{\fSpace}{\mathcal{C}(\Re^d;\Re)}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\FP}{{\sf F}}

\newcommand{\Zdim}{m}
\newcommand{\Bdim}{q}
\newcommand{\init}{\text{init}}
\newcommand{\KN}{{\sf K}^{(N)}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\xibar}{\bar{\xi}}
%\renewcommand{\v}{v}
\newcommand{\Todo}[1]{{[\color{blue} #1]}\\}

\newcommand{\inv}{^{-1}}
\newcommand{\tp}{^\transpose}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\vf}{\mathcal{I}}
\newcommand{\correct}{\mathcal{C}}
\newcommand{\grad}{\nabla}
\newcommand{\pbart}{\bar{p}_t}
\newcommand{\pt}{p_t}
\newcommand{\bij}{\psi}
\newcommand{\vfc}{\mathcal{V}}
\newcommand{\vftr}{\omega}
\newcommand{\hjb}{\mathcal{H}}
